Value Automata with Filters

We propose to study value automata with filters, a natural generalization of regular cost automata to nondeterminism. Models such as weighted automata and Parikh automata appear naturally as specializations. Results on the expressiveness of this model offer a general understanding of the behavior of the models that arise as special cases. A landscape of such restrictions is drawn.

==> define.tex <==
\makeatletter
% \def\@mathtext#1{\ensuremath{\text{#1}}\xspace}
% \def\@mathnormaltext#1{\ensuremath{\text{\normalfont#1}}\xspace}

\def\defmath#1#2{\def#1{\ensuremath{#2}\xspace}}
\def\defmathtext#1#2{%
  \edef\@@star{\csname\expandafter\@gobble\string#1 star\endcsname}
  \edef\@@nostar{\csname\expandafter\@gobble\string#1 nostar\endcsname}
  \expandafter\def\@@nostar{\text{\normalfont#2}\xspace}%
  \expandafter\def\@@star{\text{#2}\xspace}%
  \edef#1{%
    \noexpand\protect\noexpand\@ifstar%
    \unexpanded\expandafter{\@@star}
    \unexpanded\expandafter{\@@nostar}}
  }

\def\defmathsf#1#2{\defmathtext#1{\textsf{#2}}}

\defmath\timesc{\mathord{\times}c}
\defmath\plusc{\mathord{+}c}
\defmathtext\foplus{FO[+]}
\defmathtext\qfplus{$\emptyset$[+]}
\defmathsf\filt{Filter}
\defmathsf\orig{Orig}
\defmathsf\affine{Affine}
\defmathsf\scale{Scale}
\defmathsf\trans{Trans}

\defmathtext\Rc{\textsuperscript{cl}}
\defmathtext\Rcmr{\textsuperscript{cl,ml,rl}}
\defmathtext\Rcm{\textsuperscript{cl,ml}}
\defmathtext\Rcr{\textsuperscript{cl,rl}}
\defmathtext\Rm{\textsuperscript{ml}}
\defmathtext\Rmr{\textsuperscript{ml,rl}}
\defmathtext\Rr{\textsuperscript{rl}}

\defmathtext\WA{WA}
\defmathtext\UWA{UnWA}
\defmathtext\VAF{VAF}
\defmathtext\DVAF{DetVAF}
\defmathtext\UVAF{UnVAF}
\defmathtext\OVAF{OneVAF}
\defmath\semilin{\mathcal{S\!L}}
\defmath\calA{\mathcal{A}}
\defmathsf\val{val}
\defmathsf\paths{Paths}
\defmathsf\dest{Dest}
\defmath\QA{\mathcal{Q\!A}}
\defmathtext\ACz{AC$^0$}
\defmathtext\NCo{NC$^1$}
\defmathtext\ACCz{ACC$^0$}
\defmathtext\lcm{lcm}
\defmathtext\TCz{TC$^0$}
\defmath\Msol{\mathcal{M}_{\text{sol}}}
\defmathtext\FACvz{FAC$^0_{\text{v}}$}
\defmathtext\FACCvz{FACC$^0_{\text{v}}$}
\def\resp{resp.\ }
\def\kar{Klaedkte and Rueß}
\defmathsf\filter{Filt}
\defmathsf\upd{Upd}
\defmathtext\FACz{FAC$^0$}
\defmath\binal{\{0, 1\}}
\defmath\bbn{\mathbb{N}}
\defmath\bbz{\mathbb{Z}}
\defmathtext\parity{PARITY}
\defmathtext\even{EVEN}
\defmath\zed{\mathbf{z}}
\defmath\cV{\mathcal{V}}
\defmath\cG{\mathcal{G}}
\defmathtext\bV{\textbf{V}}
\defmath\eps{\varepsilon}
\def\reutschu{Reutenaeur and Sch{\"u}tzenberger\xspace}
\defmath\taus{\tau_\#}
\defmathtext\REG{REG}
\defmath\Tau{T}
\def\@refpstar#1{(\ref{#1})}
\def\@refpnostar#1{\textit{\@refpstar{#1}}}
\DeclareRobustCommand{\refp}{\@ifstar\@refpstar\@refpnostar}
\defmathtext\MOD{MOD}
\defmathtext\MAJ{MAJ}
\def\phi{\varphi}
\def\out{\mbox{:}}

\let\pipe=|
\catcode`| = 13
\newif\ifemphasize\emphasizefalse
\def|{\ifmmode\pipe\else%
  \ifemphasize%
    \global\emphasizefalse%
    \egroup%
  \else%
    \global\emphasizetrue
    \emph\bgroup
  \fi\fi}

\theorembodyfont{\normalfont}
\newtheorem{examples}{Examples}
\def\revisionset! #1 !{\gdef\therevision{#1}}
\def\revision$LastChangedRevision:#1${\revisionset!#1!}


\def\ifzero#1{%
    \@ifnextchar{0}%
      {\expandafter\@firstoftwo\remove@to@nnil}%
      {\expandafter\@secondoftwo\remove@to@nnil}%
        #1\@nnil
}
\def\ifdraft#1#2{\expandafter\ifzero\expandafter{\the\overfullrule}{#2}{#1}}
\ifdraft{%
  \usepackage{datetime}
  \global\ddmmyyyydate%
  \DeclareRobustCommand{\titleextra}{%
    \\{\normalsize Draft revision \therevision{}, compiled on \today, \currenttime}}
}{
  \DeclareRobustCommand{\titleextra}{}
}

\let\@begincompactenum\compactenum
\def\compactenum{\@minipagetrue\@begincompactenum}

\let\@begincompactitem\compactitem
\def\compactitem{\@minipagetrue\@begincompactitem}
\makeatother

